Compact Symmetric Objects -- III Evolution of the High-Luminosity Branch and a Possible Connection with Tidal Disruption Events

We use a sample of 54 Compact Symmetric Objects (CSOs) to confirm that there are two unrelated CSO classes: an edge-dimmed, low-luminosity class (CSO~1), and an edge-brightened, high-luminosity class (CSO~2). Using blind tests, we show that CSO~2s consist of three sub-classes: CSO 2.0, having prominent hot-spots at the leading edges of narrow jets and/or narrow lobes; CSO~2.2, without prominent hot-spots, and with broad jets and/or lobes; and CSO~2.1, which exhibit mixed properties. Most CSO 2s do not evolve into larger jetted-AGN, but spend their whole life-cycle as CSOs of size $\lesssim$500 pc and age $\lesssim$5000 yr. The minimum energies needed to produce the radio luminosity and structure in CSO~2s range from $\sim~10^{-4}\,M_\odot{c}^2$ to $\sim7\,M_\odot{c}^2$. We show that the transient nature of most CSO~2s, and their birthrate, can be explained through ignition in the tidal disruption events of giant stars. We also consider possibilities of tapping the spin energy of the supermassive black hole, and tapping the energy of the accretion disk. Our results demonstrate that CSOs constitute a large family of AGN in which we have thus far studied only the brightest. More comprehensive CSO studies, with higher sensitivity, resolution, and dynamic range, will revolutionize our understanding of AGN and the central engines that power them.

==> macros.tex <==
% MACROS.TEX contains generally useful macros, but not those specifically 
%            useful for paper formats.
%
\newcount\figureno  \newcount\tableno
\figureno=0         \tableno=0
%
\newbox\tablebox    \newdimen\tablewidth
%
\newbox\marginbox
\def\strutdepth{\dp\strutbox}
\def\strutheight{\ht\strutbox}
%
\def\smallformat{\hsize=5.5truein\hoffset=0.5truein
    \vsize=8truein\voffset=0.5truein\parskip=1pt}
\def\largeformat{\hsize=6.5truein\hoffset=0.0truein
    \vsize=8.5truein\voffset=0.0truein}
%
\newcount\sectionnumber \newcount\subsectionnumber 
\newcount\subsubsectionnumber
\sectionnumber=0 \subsectionnumber=0 \subsubsectionnumber=0
%
\def\secno{\ifcase\sectionnumber\or
     I\or II\or III\or IV\or V\or VI\or VII\or VIII\or IX\or
     X\or XI\or XII\fi}
\def\subsecno{\ifcase\subsectionnumber\or
     a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\fi}
\def\subsubsecno{\ifcase\subsubsectionnumber\or
     i\or ii\or iii\or iv\or v\or vi\or vii\or viii\or ix\or x\fi}
%
\def\section#1\par{\advance\sectionnumber by 1 \subsectionnumber=0
    \vskip 14pt plus 3pt minus 3pt\goodbreak
    \centerline{{\sc\secno.\ #1}}\nobreak\medskip}
\def\subsection#1\par{\advance\subsectionnumber by 1 \subsubsectionnumber=0
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\it\subsecno\/})\ {\it #1}}\nobreak\medskip}
\def\subsubsection#1\par{\advance\subsubsectionnumber by 1
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\eightrm\subsubsecno)}\ {\it #1}}\nobreak\medskip}
%
\def\today{\ifcase\month\or
    January\or February\or March\or April\or May\or June\or
    July\or August\or September\or October\or November\or December\fi
    \space\number\day, \number\year}
%
\def\sol{\ifmmode _{\mathord\odot}
         \else $_{\mathord\odot}$\fi}
\def\deg{\ifmmode ^{\circ}
         \else $^{\circ}$\fi}
\def\pdeg{\ifmmode $\setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}
          \else \setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}$\fi}
% Tony's definitions
\def\vs6{{\vskip 6pt \noindent}}
\def\vs15{{\vskip 15pt \noindent}}
%
\def\arcs{\ifmmode {^{\scriptscriptstyle\prime\prime}}
          \else $^{\scriptscriptstyle\prime\prime}$\fi}
\def\arcm{\ifmmode {^{\scriptscriptstyle\prime}}
          \else $^{\scriptscriptstyle\prime}$\fi}
\newdimen\sa  \newdimen\sb
\def\parcs{\sa=.07em \sb=.03em
     \ifmmode $\rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa$
     \else \rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa\fi}
\def\parcm{\sa=.08em \sb=.03em
     \ifmmode $\rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb$
     \else \rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb\fi}
%
\def\s#1{{\sc #1}}
\def\et{\hbox{\it et al.}}
\def\ET{{\it ET AL.}}
\def\expo#1{\ifmmode \times 10^{#1}
            \else $\times 10^{#1}$\fi}
\def\page{\vfill\eject}
\def\leaderfil{\leaders\hbox to 5pt{\hss.\hss}\hfil}
%
\def\mo{\ifmmode ^{-1}
        \else $^{-1}$\fi}
\def\sup#1{$^{\rm #1}$}
\def\mag{\sup{m}}
\def\muK{\,$\mu$\hbox{K}}
\def\,{\thinspace}
\def\tc#1{3C\,#1}
\def\dots{\relax\ifmmode \ldots
          \else $\ldots$\fi}
\def\WHzsr{\ifmmode $W\,Hz\mo\,sr\mo$
           \else W\,Hz\mo\,sr\mo \fi}
\def\mKs{\ifmmode $\,mK\,s$^{-1/2} 
         \else \,mK\,s$^{-1/2}$ \fi}
\def\microns{\ifmmode \,\mu$m$
             \else \,$\mu$m\fi}
\def\micron{\microns}

%
\def\gsim{\lower.6ex\hbox{$\buildrel>\over\sim$}}
\def\lsim{\lower.6ex\hbox{$\buildrel<\over\sim$}}
\def\ra[#1 #2 #3.#4]{#1\sup{h}#2\sup{m}#3\sup{s}\llap.#4}
\def\dec[#1 #2 #3.#4]{#1\deg#2\arcm#3\arcs\llap.#4}
\def\deco[#1 #2 #3]{#1\deg#2\arcm#3\arcs}
%
\def\refindent{\hangindent=1em \hangafter=1 \noindent}
\def\ref #1;#2;#3;#4\par{\refindent #1,{\it #2},{\bf #3},#4.\par}
\def\ajref #1;#2;#3;#4\par{\refindent #1. #2 {\bf #3},#4.\par}
\def\vref #1\par{\refindent #1.\par}
\def\cref #1;#2;#3;#4;#5\par{\refindent #1, in{\it #2}, 
                             \hbox{ed.}#3 #4, \hbox{p.} #5.\par} 
\def\bref #1;#2;#3\par{\refindent #1, {\it #2} (#3).\par}
%
%
\def\tabl #1\par{\centerline{TABLE \number\tableno}
                 \vskip 7pt
                 \centerline{#1}\nointerlineskip\noindent}
\def\endtable{\tablewidth=\wd\tablebox 
    $$\hss\copy\tablebox\hss$$
    \vskip-\lastskip\vskip -2pt}
\def\tablenote#1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=\parindent \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotenoindent #1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=0pt \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotes #1\par{
            \iftform \goodbreak\topinsert{
                 \centerline{NOTES TO TABLE \number\tableno}
                 \vskip .3cm\noindent
                 \eightpoint\input #1 }\endinsert
            \else \iftabsopen\relax
                  \else\immediate\openout\tabs=junk1\tabsopentrue\fi
                \vskip .5cm
                \centerline{NOTES TO TABLE \number\tableno} \vskip .5cm
                \immediate\write\tabs{\string\etable\space#1\string\par}
            \fi}
\def\doubleline{\vskip 3pt\hrule \vskip 1.5pt \hrule \vskip 5pt}
%
% macros for marginal stuff
%
\def\marginstuff#1{\setbox\marginbox=\vtop{
    \hsize=60pt\tolerance=10000\hbadness=10000
%    \hsize=70pt\tolerance=10000\hbadness=10000
    \parindent=0pt\eightpoint#1\par}\strut}
\def\setmarginal{\strut\vadjust{\kern-\strutdepth\kern-\ht\marginbox\vtop{%
    \moveleft 70pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%    \moveleft 80pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%
% macro for absolute positioning on a page
%
\newdimen\offset 
\newdimen\unita \newdimen\unitb
\newdimen\mina  \newdimen\minb 
%
\unita=1.0cm \mina=0.0cm
\unitb=1.0in \minb=0.0in
%
%
\def\point #1 #2 #3;{\offset=#1\unitb\advance\offset by \minb%
    \rlap{\lower\offset\hbox{\hglue #2\unitb #3}}}%
%
% macros for memos
%
\font\ssq=cmssq8 at 7pt \font\ssbx=cmssbx10 at 12pt 
\setbox0=\hbox{\ssq ATENDEES \rm\quad}
\newdimen\atndwd \atndwd=\wd0
\def\file{}
\def\memo{\hsize=5.875in \hoffset=0.3125in
    \vsize=9in     \voffset=0in
    \elevenpoint
    \vglue -0.8in
    \line{\ssq\hfil INTEROFFICE MEMORANDUM\hfil \llap{\twelvepoint\bf\file}}
    \vskip 10pt
    \centerline{\hbox to 5.4in{\ssbx C A L I F O R N I A\hskip 12pt
                I N S T I T U T E\hskip 12pt O F\hskip 12pt 
                T E C H N O L O G Y}}
    \vskip 30pt}
\def\to#1{\line{\ssq TO \rm\quad #1\hfil\today}
          \vskip 12pt}
\def\from#1{\line{\ssq FROM \rm\quad C. R. Lawrence#1\hfil
                  \ssq EXTENSION \rm\quad 4976\quad\quad
                  \ssq MAIL CODE \rm\quad 105-24}
            \vskip 12pt}
\def\subject#1{\line{\ssq SUBJECT \rm\quad#1\hfil}
               \vskip 12pt}
\def\attendees#1{\hangindent=\atndwd \hangafter=1 \noindent
                \ssq ATENDEES \rm\quad#1
                \vskip 24pt}
\def\OVRO#1{\def\file{OVRO 5m \rlap{#1-87}}}

